An asymptotic preserving method for linear systems of balance laws based on Galerkin's method

We apply the concept of Asymptotic Preserving (AP) schemes to the linearized p-system and discretize the resulting elliptic equation using standard continuous Finite Elements instead of Finite Differences. The fully discrete method is analyzed with respect to consistency, and we compare it numerically with more traditional methods such as Implicit Euler's method. Numerical results indicate that the AP method is indeed superior to more traditional methods.

==> APO_kink.tex <==
NE	eps1e4		eps1e8    eps1e1    eps1e2
2   -9.0132  -17.6021   -3.1031   -5.0197
4   -9.0195  -17.5536   -3.0786   -5.0210
8   -9.0191  -17.5430   -3.0567   -5.0182
16  -6.8060  -10.8058   -3.5500   -4.7852
32   -6.9310  -10.8747   -3.9755   -4.9158
64   -7.1651  -10.3274   -4.0939   -5.1524
128   -7.4362  -10.9200   -4.2690   -5.4244
256   -7.7229  -10.7658   -4.5137   -5.7116
512    -8.0170  -11.2890   -4.7894   -6.0044
1024  -8.3146  -11.8177   -5.0786   -6.2787
2048  -8.6140  -11.0364   -5.3740   -6.5613
4096   -8.9141  -10.9725   -5.6722   -6.8763

==> APO_time.tex <==
NE	eps1e4		eps1e8    eps1e1    eps1e2
2    0.7982    0.7982    0.7982    0.7982
4    0.7982    0.7982    0.7982    0.7982
8    0.7982    0.7982    0.7982    0.7982
16   -3.0428   -3.0428   -2.9871   -3.0493
32   -3.1484   -3.1484   -3.0058   -3.1512
64   -3.3743   -3.3743   -3.2102   -3.3752
128   -3.6416   -3.6416   -3.4979   -3.6415
256   -3.9266   -3.9266   -3.8097   -3.9260
512   -4.2198   -4.2198   -4.1186   -4.2190
1024  -4.5170   -4.5170   -4.4229   -4.5160
2048  -4.8161   -4.8161   -4.7250   -4.8150
4096  -5.1162   -5.1162   -5.0264   -5.1151

==> AP_kink.tex <==
NE	eps1e4		eps1e8    eps1e1    eps1e2
2   	-9.2746		-17.6021	-3.1673		-5.2613
4   	-9.0817		-17.5536	-3.0306		-5.0729
8   	-9.0345		-17.5430	-3.0135		-5.0284
16   	-9.8413		-17.8415	-3.4351		-5.8425
32  	-10.1372	-18.1419	-3.8710		-6.1386
64  	-10.4334	-9.85770	-4.2393		-6.4349
128  	-10.7316	-10.1587	-4.5130		-6.7331
256  	-11.0309	-9.4597		-4.7853		-7.0326
512  	-11.3312	-8.65368	-5.0705		-7.3224
1024  	-11.6316	-10.7608	-5.3633		-7.3706
2048  	-11.9170	-9.3136		-5.6602		-7.5243
4096	-12.2289	-9.8378		-5.9591		-7.9888

==> AP_time.tex <==
NE	eps1e4		eps1e8    eps1e1    eps1e2
2    	0.7982		0.7982    0.7982    0.7982
4    	0.7982    	0.7982    0.7982    0.7982
8    	0.7982    	0.7982    0.7982    0.7982
16   	-9.4448   	-8.0515   -3.4403   -5.4498
32   	-7.7371   	-8.3524   -3.5806   -5.5853
64   	-7.7935   -8.9540   -3.8084   -5.7280
128   	-7.9972   -9.0443   -4.2072   -5.9512
256   	-8.2540   -8.9829   -4.6791   -6.2146
512   	-8.5338   -8.9438   -5.1116   -6.4972
1024	 -8.8244   -8.7362   -5.4734   -6.7891
2048   -9.1203   -9.7201   -5.7942   -7.0841
4096   -9.4188   -9.0068   -6.1006   -7.3592


==> IE_kink.tex <==
NE	eps1e4		eps1e8    eps1e1    eps1e2
2   	-8.1801		-4.6647		-2.6287		-4.1871		 -8.6637
4   	-8.8455		-4.3379		-3.0687		-4.8611		 -9.587
8   	-8.9727		-4.1825		-3.4476		-5.2360		  -6.499
16   	-9.3371		-4.5061		-3.7268		-5.3462		   -5.8409
32   	-9.3310		-5.1269		-4.0199		-5.4219	 	   -6.3420	   
64   	-9.4134		-3.9639		-4.3101		-5.5245		    -6.4353
128   	-9.4290		-3.2847		-4.5958		-5.7430		     -6.0163
256   	-9.4355		-2.7887		-4.8845		-6.1184		      -5.9421  
512   	-9.4400		-2.7853		-5.1780		-6.5608		       -6.0602
1024   	-9.4438		-2.6960		-5.4747		-7.007
2048	-9.4531		-3.9966		-5.7735		-7.4523
4096	-9.4856		-2.8568		-6.0733		-7.8982


==> IE_time.tex <==
NE	eps1e4		eps1e8    eps1e1    eps1e2
2    0.7982    0.7981    0.7982    0.7982
4    0.7970    0.7950    0.7973    0.7970
8    0.7977    0.8044    0.7977    0.7977
16   -2.5554   -1.7662   -2.5694   -2.5556
32   -2.9247   -2.2936   -2.9321   -2.9249
64   -3.2648   -3.2734   -3.2670   -3.2650
128   -3.5872   -2.8067   -3.5866   -3.5873
256   -3.8994   -2.7578   -3.8977   -3.8996
512   -4.2062   -3.3280   -4.2041   -4.2063
1024   -4.5102   -2.8723   -4.5079   -4.5102
2048   -4.8127   -3.0016   -4.8104   -4.8127
4096   -5.1145   -2.9536   -5.1121   -5.1145

